An Architecture for In-Vehicle Network

As vehicles get equipped with increasingly complex sensors and processors, the communication requirements become more demanding. Traditionally, vehicles have used specialized networking technologies designed to guarantee bounded latencies, such as the Controller Area Network (CAN) bus. Recently, some have used dedicated technologies to transport signals from cameras, lidars, radars, and ultrasonic sensors. In parallel, IEEE working groups are defining Ethernet standards for time-sensitive networks (TSN). This paper describes an Ethernet-based architecture with provable guaranteed performance and simple configuration that is suitable for supporting the communication requirements of many vehicles.

==> bibliography.tex <==

%----------------------------------------------------------------------------------------
%	REFERENCES
%----------------------------------------------------------------------------------------
\newpage
\begin{thebibliography}{00}

	\addcontentsline{toc}{section}{References}

	% --- MOTIVATION ---

	\bibitem{lee} Lee, Youngwoo, and KyoungSoo Park. 
	"Meeting the real-time constraints with standard Ethernet in an in-vehicle network." 
	In 2013 IEEE Intelligent Vehicles Symposium (IV), pp. 1313-1318. IEEE, 2013.
	% (available at \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=6629648}{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=6629648})

	\bibitem{steinbach} Steinbach, Till, Hyung-Taek Lim, Franz Korf, Thomas C. Schmidt, Daniel Herrscher, and Adam Wolisz. 
	"Beware of the hidden! How cross-traffic affects quality assurances of competing real-time Ethernet standards for in-car communication." 
	In 2015 IEEE 40th Conference on Local Computer Networks (LCN), pp. 1-9. IEEE, 2015.
	% (available at \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7366277}{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=7366277})

	\bibitem{zinner}
	H. Zinner, J. Brand, D. Hopf.
	"Automotive E/E Architecture evolution and the impact on the network",
	March 2019, 
	(available at \href{http://ieee802.org/1/files/public/docs2019/dg-zinner-automotive-architecture-evolution-0319-v02.pdf}
	{http://ieee802.org/1/files/public/docs2019/dg-zinner-automotive-architecture-evolution-0319-v02.pdf})

	\bibitem{cisco} Cisco. "Time-Sensitive Networking: A Technical Introduction" \\
	(available at \href{https://www.cisco.com/c/dam/en/us/solutions/collateral/industry-solutions/white-paper-c11-738950.pdf}{https://www.cisco.com/c/dam/en/us/solutions/collateral/industry-solutions/white-paper-c11-738950.pdf})

	\bibitem{tsn} 
	Institute of Electrical and Electronics Engineers, Inc., 
	“IEEE 802.1 Time Sensitive-Networking Task Group.” 
	\href{http://www.ieee802.org/1/pages/tsn.html}{http://www.ieee802.org/1/pages/tsn.html}

	% --- OBJECTIVE ---

	\bibitem{OMNeT}
	A. Varga. OMNeT++: an extensible, modular, component-based C++ simulation library and framework. (available at \href{https://omnetpp.org/}{https://omnetpp.org/})

	\bibitem{NeSTiNg}
	J. Falk, D. Hellmanns, B. Carabelli et al. 
	“NeSTiNg: Simulating IEEE Time-sensitive Networking (TSN) in OMNeT++”. 
	In: Proceedings of the 2019 International Conference on Networked Systems (NetSys). Garching b. München, Germany, Mar. 2019.
	(available at \href{ftp://ftp.informatik.uni-stuttgart.de/pub/library/ncstrl.ustuttgart_fi/INPROC-2019-04/INPROC-2019-04.pdf}{ftp://ftp.informatik.uni-stuttgart.de/pub/library/ncstrl.ustuttgart\_fi/INPROC-2019-04/INPROC-2019-04.pdf})\\
	(sourcecode at \href{https://gitlab.com/ipvs/nesting}{https://gitlab.com/ipvs/nesting})

	% --- RELATED ---

	\bibitem{ULL Overview}
	Nasrallah, Ahmed, Akhilesh S. Thyagaturu, Ziyad Alharbi, Cuixiang Wang, Xing Shao, Martin Reisslein, and Hesham ElBakoury. "Ultra-low latency (ULL) networks: The IEEE TSN and IETF DetNet standards and related 5G ULL research." IEEE Communications Surveys \& Tutorials 21, no. 1 (2018): 88-145.

	\bibitem{Queck}
	Queck, Rene. "Analysis of Ethernet AVB for automotive networks using Network Calculus." In 2012 IEEE International Conference on Vehicular Electronics and Safety (ICVES 2012), pp. 61-67. IEEE, 2012.

	\bibitem{Zhao CBS TAS}
	Zhao, Luxi, Paul Pop, Zhong Zheng, and Qiao Li. "Timing analysis of AVB traffic in TSN networks using network calculus." In 2018 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS), pp. 25-36. IEEE, 2018.

	\bibitem{Boudec CBS}
	Mohammadpour, Ehsan, Eleni Stai, and Jean-Yves Le Boudec. "Improved Credit Bounds for the Credit-Based Shaper in Time-Sensitive Networking." arXiv preprint arXiv:1901.04957 (2019).

	\bibitem{UBS} Specht, Johannes, and Soheil Samii. "Urgency-based scheduler for time-sensitive switched ethernet networks." In 2016 28th Euromicro Conference on Real-Time Systems (ECRTS), pp. 75-85. IEEE, 2016.

	\bibitem{Boudec ATS}
	Mohammadpour, Ehsan, Eleni Stai, Maaz Mohiuddin, and Jean-Yves Le Boudec. "Latency and Backlog Bounds in Time-Sensitive Networking with Credit Based Shapers and Asynchronous Traffic Shaping." In 2018 30th International Teletraffic Congress (ITC 30), vol. 2, pp. 1-6. IEEE, 2018.

	\bibitem{ATS Zhou}
	Zhou, Zifan, Ying Yan, Michael Berger, and Sarah Ruepp. "Analysis and modeling of asynchronous traffic shaping in time sensitive networks." In 2018 14th IEEE International Workshop on Factory Communication Systems (WFCS), pp. 1-4. IEEE, 2018.

	\bibitem{specht2017}
	Specht, Johannes, and Soheil Samii. "Synthesis of queue and priority assignment for asynchronous traffic shaping in switched Ethernet." In 2017 IEEE Real-Time Systems Symposium (RTSS), pp. 178-187. IEEE, 2017.

	\bibitem{resource-efficient}
	Rahmani, Mehrnoush, Ktawut Tappayuthpijarn, Benjamin Krebs, Eckehard Steinbach, and Richard Bogenberger. "Traffic shaping for resource-efficient in-vehicle communication." IEEE Transactions on Industrial Informatics 5, no. 4 (2009): 414-428. 
	% (available at \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=4926124}{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=4926124})

	% --- TSN ---

	\bibitem{MEF} MEF Technical Specification 10.3 (MEF 10.3), Ethernet Service Attributes Phase 3 \\
	(available at \href{https://www.mef.net/Assets/Technical_Specifications/PDF/MEF_10.3.pdf}{https://www.mef.net/Assets/Technical\_Specifications/PDF/MEF\_10.3.pdf})

	\bibitem{IEEE-ATS} IEEE802.1 TSN Task Group, "IEEE802.1Qcr - Asynchronous Traffic Shaper" \\ 
	(available at \href{http://www.ieee802.org/1/pages/802.1cr.html}{http://www.ieee802.org/1/pages/802.1cr.html})

	\bibitem{UBS xtraffic}
	Johannes Specht "Urgency Based Scheduler - AVB Gen. 1 worst case with subshapers" 02.12.2013
	(availalbe at
	\href{http://grouper.ieee.org/groups/802/1/files/public/docs2013/new-tsn-specht-ubs-avb1case-1213-v01.pdf}{http://grouper.ieee.org/groups/802/1/files/public/docs2013/new-tsn-specht-ubs-avb1case-1213-v01.pdf})

	\bibitem{IEEE-CBS} IEEE802.1 TSN Task Group, "IEEE802.1Qav - Forwarding and Queuing Enhancements for Time-Sensitive Streams" 
	(available at \href{http://www.ieee802.org/1/pages/802.1av.html}{http://www.ieee802.org/1/pages/802.1av.html})

	\bibitem{CBS-Sensor} He, Feng, Lin Zhao, and Ershuai Li. "Impact analysis of flow shaping in Ethernet-AVB/TSN and AFDX from network calculus and simulation perspective." Sensors 17, no. 5 (2017): 1181.

	\bibitem{IEEE-TAS} IEEE802.1 TSN Task Group, "IEEE802.1Qbv - Enhancements for Scheduled Traffic" \\ 
	(available at \href{http://www.ieee802.org/1/pages/802.1bv.html}{http://www.ieee802.org/1/pages/802.1bv.html})

	\bibitem{IEEE-AS} IEEE, "802.1AS - Timing and Synchronization" 
	(available at \href{http://www.ieee802.org/1/pages/802.1as.html}{http://www.ieee802.org/1/pages/802.1as.html})

	% \bibitem{IEEE-Qbu} IEEE802.1 TSN Task Group, "IEEE802.1Qbu - Frame Preemption" \\ (available at \href{http://www.ieee802.org/1/pages/802.1bu.html}{http://www.ieee802.org/1/pages/802.1bu.html})
	
	\bibitem{IEEE-CQF} IEEE802.1 TSN Task Group, "P802.1Qch – Cyclic Queuing and Forwarding" \\ 
	(available at \href{https://1.ieee802.org/tsn/802-1qch/}{https://1.ieee802.org/tsn/802-1qch/})

	\bibitem{IEEE-SRP} IEEE, "802.1Qat - Stream Reservation Protocol" \\ 
	(available at \href{http://ieee802.org/1/pages/802.1at.html}{http://ieee802.org/1/pages/802.1at.html})

	% --- TRAFFIC TYPES ---

	\bibitem{IEEE-PTP}
	IEEE-1588 "Standard for a Precision Clock Synchronization Protocol for Networked Measurement and Control Systems"

	\bibitem{Garner} 
	Geoffrey M. Garner, 
	Time Stamp Accuracy needed by 802SIEEE 802.1AS, 
	January 6, 2009 \\
	(available at \href{http://www.ieee802.org/1/files/public/docs2008/as-garner-timestamp-accuracy-0109.pdf}{http://www.ieee802.org/1/files/public/docs2008/as-garner-timestamp-accuracy-0109.pdf})

	\bibitem{limitMTU} Lee, Youngwoo, and KyoungSoo Park. "Meeting the real-time constraints with standard Ethernet in an in-vehicle network." In 2013 IEEE Intelligent Vehicles Symposium (IV), pp. 1313-1318. IEEE, 2013.

	\bibitem{Lim1}
	Lim, Hyung-Taek, Kay Weckemann, and Daniel Herrscher. "Performance study of an in-car switched ethernet network without prioritization." In International Workshop on Communication Technologies for Vehicles, pp. 165-175. Springer, Berlin, Heidelberg, 2011.

	\bibitem{Lim2}
	Lim, Hyung-Taek, Lars Völker, and Daniel Herrscher. "Challenges in a future IP/Ethernet-based in-car network for real-time applications." In Proceedings of the 48th Design Automation Conference, pp. 7-12. ACM, 2011.

	% --- SHAPING ---

	\bibitem{shaping-rfc} % intro
	Blake, S., D. Black, M. Carlson, E. Davies, Z. Wang, and W. Weiss. 
	"RFC 2475: An architecture for differentiated services." December 1998.
	(available at \href{https://tools.ietf.org/html/rfc2475#section-2.3.3.3}{https://tools.ietf.org/html/rfc2475})

	\bibitem{TUM-guide} %PBOO
	Van Bemten, Amaury, and Wolfgang Kellerer. "Network calculus: A comprehensive guide." (2016).
	(available at \href{https://mediatum.ub.tum.de/doc/1328613/file.pdf#page=41}{https://mediatum.ub.tum.de/doc/1328613/file.pdf})

	% --- GATING ---

	\bibitem{Craciunas16} % SMT
	Craciunas, Silviu S., Ramon Serna Oliver, Martin Chmelík, and Wilfried Steiner. "Scheduling real-time communication in IEEE 802.1 Qbv time sensitive networks." In Proceedings of the 24th International Conference on Real-Time Networks and Systems, pp. 183-192. ACM, 2016.

	\bibitem{TSSDN} % ILP
	Nayak, Naresh Ganesh, Frank Dürr, and Kurt Rothermel. "Time-sensitive software-defined network (TSSDN) for real-time applications." In Proceedings of the 24th International Conference on Real-Time Networks and Systems, pp. 193-202. ACM, 2016.

	\bibitem{NOWAIT}
	Dürr, Frank, and Naresh Ganesh Nayak. "No-wait packet scheduling for IEEE time-sensitive networks (TSN)." In Proceedings of the 24th International Conference on Real-Time Networks and Systems, pp. 203-212. ACM, 2016.

	\bibitem{RTaW schedulability}
	Mai, Tieu Long, Nicolas Navet, and Jörn Migge. "On the use of supervised machine learning for assessing schedulability: application to Ethernet TSN." In 27th International Conference on Real-Time Networks and Systems (RTNS 2019). 2019.

	\bibitem{Thangamuthu15}
	Thangamuthu, Sivakumar, Nicola Concer, Pieter JL Cuijpers, and Johan J. Lukkien. "Analysis of ethernet-switch traffic shapers for in-vehicle networking applications." In Proceedings of the 2015 Design, Automation \& Test in Europe Conference \& Exhibition, pp. 55-60. EDA Consortium, 2015.

\end{thebibliography}

Unless otherwise stated, URLs were last checked on \today.
